An Oblivious Spanning Tree for Buy-at-Bulk Network Design Problems

We consider the problem of constructing a single spanning tree for the single-source buy-at-bulk network design problem for doubling-dimension graphs. We compute a spanning tree to route a set of demands (or data) along a graph to or from a designated root node. The demands could be aggregated at (or symmetrically distributed to) intermediate nodes where the fusion-cost is specified by a non-negative concave function $f$. We describe a novel approach for developing an oblivious spanning tree in the sense that it is independent of the number of data sources (or demands) and cost function at intermediate nodes. To our knowledge, this is the first paper to propose a single spanning tree solution to this problem (as opposed to multiple overlay trees). There has been no prior work where the tree is oblivious to both the fusion cost function and the set of sources (demands). We present a deterministic, polynomial-time algorithm for constructing a spanning tree in low doubling graphs that guarantees $\log^{3}D\cdot\log n$-approximation over the optimal cost, where $D$ is the diameter of the graph and $n$ the total number of nodes. With constant fusion-cost function our spanning tree gives a $O(\log^3 D)$-approximation for every Steiner tree to the root.

==> Algorithm.tex <==
\section{Data Fusion Algorithm}
\label{section:fusion-algorithm}


\begin{comment}

\begin{algorithm}[t]
\linesnumbered
\SetLine
\KwIn{A virtual tree $T_v$ 
with $\kappa$ levels oriented toward sink node $s$; 
a concave non-decreasing cost fusion function $f$}
\KwOut{Fused data at sink $s$.}
\BlankLine
Divide time into phases where each phase consists of $\kappa$ rounds;
the duration of each round $i$, where $1 \leq i \leq \kappa$,
is proportional to the time needed to transfer data from level $i - 1$ to level $i$ of $T_v$.

\For{each phase} {
Source sensors send their data to the respective leaders at level 1.

\For{each round $i = 1, \ldots, \kappa$} {
If a leader at level $i-1$ has data, then it sends its data to the
respective parent at level $i$ (unless the parent is the node itself).

The leaders of level $i$ fuse the received data and the size of the output data is determined 
by the fusion function $f$.
}
}
\caption{Data Fusion Algorithm}
\label{alg:data-fusion}
\end{algorithm}

\end{comment}




==> Discussion.tex <==
\section{Discussion}

In the virtual tree $T_v$, there may be occurances where two or more paths either intersect (that are modified as virtual paths if the paths do not belong to the same level) or merge at some point to reach a common destination. The current analysis treats these paths as separate paths. It would be better (more efficient) if the analysis considers the merged segment as a common path segment where the fused data propagates. 


\subsection{Timings and Path Activation}
	Each node along a path $p_i$ is assigned a time-slot to send its information downstream to its leader. The assignment of time slots are given in the following way:
	\begin{enumerate}
		\item Number of nodes in the path is computed.
		\item The end-node at the lower-level is given the first time-slot and 
		the other end-node (destination) which is at a higher-level is given 
		the last time-slot.
		\item The intermediate nodes are given incremental slots by 1.
	\end{enumerate}

If there are $n$ nodes, the $n^{th}$ node (destination node) gets time-slot $n$. Typically, if the first node has data to send, it sends data at time-slot $1$ and that path-segment in $p_i$ gets activated (not the whole path). When the second node gets this data, it will fuse its own data (if it has one) and relays this data during time-slot $2$. If $(n-k)^{th}$ node has data to send, it has to wait for $k$ time-slots before it can send its own data downstream. Suppose at time $(n-k)$, it gets data from upstream, it will fuse its own data and send it downstream. 

\subsection{Path Segments and Node Roles}

Consider a path $p_i^j$ with $n$ nodes. When an end-node sends data to its leader, the data is relayed and fused along multiple nodes along the path. Each of those intermediate nodes will play its role as $i$-level nodes. If the same path is intersected by $p_k^j$, some of the nodes in $p_i^j$ will have to play dual roles (fuse and relay data for both $i$-level data and for $k$-level data). Likewise, a node in a path could have multiple roles, depending on the number of intersections. Such roles of nodes dictate the multiple time-schedules for them. Such multiple-role-nodes would have to abide by different time-schedules to fuse and relay data that flows in different level paths.

\begin{observation}
The data fusion process in the virtual tree $T_v$ is not as efficient when compared to that of the constructed spanning tree $T_s$.
\end{observation}

In a virtual path of a $T_v$, data briefly traverses against the normal direction of flow to the sink. This is due to the presence of pseudo-leader that lies against the normal direction of flow. On the contrary, the spanning tree $T_s$ doesn't exhibit this problem as the data at the intersection would wait there until data from upstream fuses with it or for its time slot to begin forwarding data downstream. Hence, in $T_s$, data will never traverse upstream (and then downstream) like in $T_v$.

